CorrDetector: A Framework for Structural Corrosion Detection from Drone Images using Ensemble Deep Learning

In this paper, we propose a new technique that applies automated image analysis in the area of structural corrosion monitoring and demonstrate improved efficacy compared to existing approaches. Structural corrosion monitoring is the initial step of the risk-based maintenance philosophy and depends on an engineer's assessment regarding the risk of building failure balanced against the fiscal cost of maintenance. This introduces the opportunity for human error which is further complicated when restricted to assessment using drone captured images for those areas not reachable by humans due to many background noises. The importance of this problem has promoted an active research community aiming to support the engineer through the use of artificial intelligence (AI) image analysis for corrosion detection. In this paper, we advance this area of research with the development of a framework, CorrDetector. CorrDetector uses a novel ensemble deep learning approach underpinned by convolutional neural networks (CNNs) for structural identification and corrosion feature extraction. We provide an empirical evaluation using real-world images of a complicated structure (e.g. telecommunication tower) captured by drones, a typical scenario for engineers. Our study demonstrates that the ensemble approach of \model significantly outperforms the state-of-the-art in terms of classification accuracy.

==> system_arch.tex <==
\section{Architecture of the CorrDetector Framework}
\label{sec:architecture}

The architecture of \model framework is illustrated in Figure \ref{fig:architecture}. It consists of four main layers: \textit{Data acquisition}, \textit{Data preparation}, \textit{Data analysis} and \textit{Decision layer}. The detailed description of these layers is provided below.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=4.5in]{images/architecture.png}
    \caption{The architecture of the \model framework}
    \label{fig:architecture}
\end{figure}

\subsection{Data acquisition layer}
A large collection of images is essential to properly train a deep learning classifier. In this layer, a large number of images of the targeted industrial structure (e.g. building roofs, telecommunication towers, bridges, poles, wires and pipelines) are acquired. The main driver of this layer is human-operated drones with advanced cameras which capture images at the level of detail that was not possible earlier. These drones fly up-close to the industrial structures and take a large number of high-resolution images (e.g. 5820 X 3952) from multiple angles, positions and different lighting conditions for each asset. Using these images, engineers identify areas of defects (e.g. corrosion) by visual inspection. The human expert annotated images are utilised in the next layer to identify the training data set required for model training. Some samples of telecommunication tower images captured by drones are shown in Figure \ref{fig:drone_images}.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=4.5in]{images/drone_images.png}
    \caption{Example images captured in the data acquisition layer}
    \label{fig:drone_images}
\end{figure}

\subsection{Data preparation layer}

Once a large number of images are captured by multiple drones in the data acquisition layer, they are stored in a centralised location. These images are then annotated with the help of human experts using various annotation software tools. \model incorporates two types of annotations in this layer. Given an image, the first type is the \textit{grid-based annotation} where the multiple small rectangular grids (or segments)~\footnote{In this paper, to simplify the presentation, we interchangeably use the terms, grid and segment.} in the image are drawn. Then, a human expert annotates each of these grids with corrosion or non-corrosion, depending on the fact that the grid contains corroded structural component(s) (see Figure \ref{fig:annotation}(a)). The grids are separated using image processing techniques. These annotations are used to build ground truth information for corrosion detection deep learning model in \model.

Another type of the annotation is the \textit{object annotation}, where a human expert uses an image annotation tool to create a polygonal mask annotation around the target object (e.g. a telecommunication tower on which corrosion needs to be detected). The annotated data are used to train an object recognition model in \model. This type of the annotation is used to separate the target object from other background (see Figure \ref{fig:annotation}(b)) information present in the unaltered drone images. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=4.5in]{images/annotation.png}
    \caption{Example of an image annotation by a human expert using annotation tools}
    \label{fig:annotation}
\end{figure}

\subsection{Data analysis layer}
% The major functionalities of this layer is image processing, deep learning model development, model training and validation. In this layer, the training images are first processed prepared to train our learning model. Multiple CNN models including some state-of-the-art models are developed and trained with various parameter configurations. Separate CNN models are used for grid-based corrosion detection and industrial object identification. Each model is validated with a separate validation set. Once a satisfactory validation level is achieved all models are saved. An image grid aggregator is used to combine all segmented grids within an image to decide about image level corrosion. Another machine learning model takes the output produced by two CNN models for corrosion and object detection as input and uses an ensemble approach to generate the final model.

In this layer, two deep learning models using different CNNs are learned that will be used to develop an ensemble model in \model.
%The major functionalities of this layer is image processing and deep learning model development. In this layer, the training images are used to train our learning model. 
These models are denoted as $\modelname_c$ and $\modelname_o$ that will be used for grid-based corrosion detection and industrial object identification, respectively (details of these models are presented in Section \ref{sec:method}). The \textit{image grids aggregator} is used to combine all segments (or grids) within the target image to predict whether there is corrosion or not in the image. As another key model, \model also incorporates, an ensemble model, denoted as $\modelname$, that takes the outputs predicted by the $\modelname_c$ and $\modelname_o$ as the input, and predict which structural objects has corrosion or not. This ensemble approach aims to improve our prediction capability by predicting corrosion on only the structural components.

%another machine learning method takes the output produced by the two CNN models for corrosion and object detection as input and uses an ensemble approach to build the final model for prediction about corrosion.

\subsection{Decision layer}
This is the classification layer that makes the final two decisions for a given unknown image. The first decision is the outcome that contains corrosion or not in the image. The decision is made by aggregating outcomes of individual segments estimated using $\lambda_c$ for that image. The other decision is about which regions of industrial object are likely to have corrosion in the image. This is done using the ensemble model, $\lambda$. The corrosion regions can be visualised as highlighted rectangular grids. 


